Theoretical Analysis of the Energy Capture in Strictly Bandlimited Ultra-Wideband Channels

The frequency selectivity of wireless communication channels can be characterized by the delay spread Ds of the channel impulse response. If the delay spread is small compared to the bandwidth W of the input signal, that is, Ds*W approximately equal to 1, the channel appears to be flat fading. For Ds*W >> 1, the channel appears to be frequency selective, which is usually the case for wideband signals. In the first case, small scale synchronization with a precision much higher than the sampling time T = 1/W is crucial. In this paper, it is shown by analytical means that this is different in the wideband regime. Here synchronization with a precision of T is sufficient and small scale synchronization cannot further increase the captured energy at the receiver. Simulation results show that this effect already occurs for W > 50MHz for the IEEE 802.15.4a channel model.

==> Makefile <==
PROJECT=iswcs08
TMPFILES=*.aux *.bak *.bbl *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps

default: $(PROJECT).tex

clean:
	rm -f $(TMPFILES);
clean_pdf:
	rm -f $(PROJECT).pdf;

$(PROJECT).tex: clean_pdf
	pdflatex $(PROJECT);

$(PROJECT).texAll: clean
	ps4pdf $(PROJECT);
	pdflatex $(PROJECT);
	bibtex $(PROJECT);
	pdflatex $(PROJECT);
	pdflatex $(PROJECT);
	pdflatex $(PROJECT);

bib:	
	bibtex $(PROJECT);

literatur:
	cp ~/Desktop/work/freia/references/trunk/Literatur.bib ./;
	cp ~/Desktop/work/freia/references/trunk/confs-jrnls.bib ./;

final: clean clean_pdf literatur
	latex $(PROJECT).tex;
	latex $(PROJECT).tex;
	bibtex $(PROJECT);
	latex $(PROJECT).tex;
	latex $(PROJECT).tex;
	dvips -o $(PROJECT).ps $(PROJECT).dvi;
	ps2pdf14 -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $(PROJECT).ps;
	pdffonts $(PROJECT).pdf;

